A Privacy-Preserving Platform for Recording COVID-19 Vaccine Passports

Digital vaccine passports are one of the main solutions which would allow the restart of travel in a post COVID-19 world. Trust, scalability and security are all key challenges one must overcome in implementing a vaccine passport. Initial approaches attempt to solve this problem by using centralised systems with trusted authorities. However, sharing vaccine passport data between different organisations, regions and countries has become a major challenge. This paper designs a new platform architecture for creating, storing and verifying digital COVID-19 vaccine certifications. The platform makes use of the InterPlanetary File System (IPFS) to guarantee there is no single point of failure and allow data to be securely distributed globally. Blockchain and smart contracts are also integrated into the platform to define policies and log access rights to vaccine passport data while ensuring all actions are audited and verifiably immutable. Our proposed platform realises General Data Protection Regulation (GDPR) requirements in terms of user consent, data encryption, data erasure and accountability obligations. We assess the scalability and performance of the platform using IPFS and Blockchain test networks.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> consentmodel.tex <==
\subsection{Consent models}
Liang et al \cite{liang2017integrating} used Hyperledger Fabric to share consent information, as illustrated in Figure \ref{jain}. With this a user could share healthcare information with insurance companies, in order to get an insurance quote. On a data sharing event, an event record is created as a tuple of {recordhash, owner, receiver, time, location, expiry-date, signature}, and submitted to the blockchain network in order to convert health records into a transaction. Every action on the health record is then recorded and is thus accountable. The research project uses Hyperledger Fabric membership service component and the channel scheme, and uses:

\begin{itemize}
\item Membership service provider (CA). The CA focuses on membership enrollment. Each participating node is issued with enrollment certiﬁcates and transaction certiﬁcates for the network and create the access control list during channel establishment
\item Chaincode. This is the code responsible for the deploy, invoke and query transactions, and isolates each of the participating parties in the network.
\end{itemize}

License accoUntability and CompliancE (LUCE) data sharing platform built on the Ethereum platform \cite{havelange2019luce}. It allows citizens to rectify and erase data in relation to General Data Protection Regulation's (GDPR) rights. LUCE tracks data in terms of licensing terms and has three core roles: Data Providers, Data Requesters, and Supervisory Authorities (Figure \ref{luce1}). Figure \ref{luce2} provides an outline of the architecture, and where we have states of:

\begin{itemize}
\item Sharing document: publish.
\item Accessing dataset: query, request, accessing terms, accepting licensing terms, and download token.
\item Monitoring compliance: access token, access data, reports compliance, access token, replication and checking compliance.
\item GDPR compliance: rights to access; rights to erase and right to rectification; and supervisory authority.
\end{itemize}

\begin{figure}[h!]
\includegraphics[width=0.95\linewidth]{figures/luce1.png}
\caption{LUCE roles \cite{havelange2019luce}}
\label{luce1}
\end{figure}

\begin{figure}[h!]
\includegraphics[width=0.95\linewidth]{figures/luce2.png}
\caption{LUCE architecture \cite{havelange2019luce}}
\label{luce2}
\end{figure}

Jaiman et al \cite{jaiman2020consent} created a blockchain-based data-sharing consent model for health data, and where smart contracts represent a citizen's consent over their health data. It uses two ontologies defined within the Ethereum blockchain (Figure \ref{jain3}): 

\begin{itemize}
\item Data Use Ontology (DUO). This defines citizen consent.
\item Automatable Discovery and Access Matrix (ADA-M). This defines the formatting of queries from data requesters. 
\end{itemize}

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.95\linewidth]{figures/jai.png}
\caption{Hyperledger to share consent information \cite{liang2017integrating}}
\label{jain}
\end{center}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.95\linewidth]{figures/jaima3.gif}
\label{jain3}
\caption{Ethereum data-sharing consent model \cite{jaiman2020consent}}
\end{center}
\end{figure}

\subsubsection{Right to be forgotten}\label{sect:5.1}
Politou et al \cite{politou2020delegated} define the Right to be Forgotten (RtbF) as requirement of GDPR, and thus for data to be erased. Unfortunately, enforcing this across the entire IPFS network is not actually feasible. They implemented an anonymous protocol for delegated content erasure requests within IPFS, and where erasure is only allowed by the original content provider or their delegates. Figure \ref{erase} provides an overview of the system.

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.95\linewidth]{figures/erase.png}
\label{erase}
\caption{Erasure in IPFS \cite{politou2020delegated}}
\end{center}
\end{figure}



==> ipfs.tex <==

\subsection{InterPlanetary File System}
The IPFS (InterPlanetary File System) implements a distributed infrastructure using P2P methods, and where there is no centralised server. As with Torrent networks, it is defined as being censorship-resistant \cite{henningsen2020mapping}. Benet \cite{benet2014ipfs} outlines that IPFS can be likened to the Web where we use content-address hyperlinks, but where a single BitTorrent swarm exchange objects within one Git repository. 

IPFS breaks files up into blocks or chunks and traces and uses a Merkle DAG (Direct Acyclic Graph) to define the version control of files and a distributed hashtable.  Within a traditional blockchain infrastructure we sequentially store transactions. This can take some time to create a consensus through the building of blocks. With a DAG, each of the transactions becomes a block, and it thus speeds up the consensus mechanisms. Sergio Demian Lerner \cite{lerner2015dagcoin} outlined that in a DAG there were no fixed blocks, and that each transaction brings with it, its own proof of work. Within this he defined the usage of a fast cache for the most recent transactions, and where older transactions cannot be used as a reference.

\subsubsection{Architecture}
Chen et al \cite{chen2017improved},  as shown in Figure \ref{chen}, define four core layers for storage (Layer 4), routing (Layer 3), virtual chain (Layer 2), and blockchain (Layer 1).  Within the blockchain layer, it is possible to build a new blockchain or use Bitcoin's blockchain. A significant and prominently distributed database technology that elaborates the blockchain technology is Blockstack \cite{ali2017blockstack}. Blockstack operates by default using the Gaia distributed database that is able to store its data decentralized in the users' web browsers instead of a centralized web server, thus enhancing privacy. Blockstack recently released Stacks 2.0 which is built on top of the Bitcoin blockchain, in order to utilise smart contracts and decentralised applications \cite{ali2020stacks}.

%The Blockstack framework is currently built on the Bitcoin blockchain, but can be moved onto another platform. 

For the virtual chain layer, the transactions are processed and verified, and then sent to the blockchain layer to be stored.  Each transaction must have been signed by the private key of a sender, and these are verified by their public key. Typically transactions are for a node to bind its IP address and its associated account (such as defined by its public key), and also one to declare the files that it is associated with. Files can either be \textbf{long-term immutable} or  \textbf{occasionally mutable}, and are broken into blocks to be bartered in the BitSwap protocol. Each of the blocks are then identified with a \textbf{content identifier (CID)}. With the \textbf{Bitswap protocol} nodes distribute \textit{want-lists} to their peers, and contains the list of CIDs for blocks that they want to receive. Each node remembers which blocks its peers want. Whenever a node receives a block it checks its list to see if one of its connected peers wanted the received block. The BitSwap protocol involves a node having two lists: the blocks they want; and the blocks they have. Nodes thus barter between themselves. Within a BitTorrent exchange, the data is exchanged in a single torrent.

The routing layer extracts the information from Layer 2 and maps the routing address of an account to their associated files or blocks under their account. The storage layer (Layer 4) is where the data itself is stored (mutable storage and immutable storage).  In \cite{chen2017improved}, the authors make  improvements to IPFS by adding a zig-zag file storage structure in order to provide a triple replication scheme (for frequently used data) and for an erasure codes storage scheme (for infrequency used data). The authors define that the method can differentiate between hot data and cold data. Within hot data storage we store data near the computation and where there is fast access to the data, whereas cold data can be store within a cloud storage.


\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.95\linewidth]{figures/chen01.gif}
\caption{IPFS Architecture \cite{chen2017improved}}
\label{chen}
\end{center}
\end{figure}

\subsubsection{IoT integration}
Muralidharan et al \cite{muralidharan2019interplanetary} implemented an IoT network using IPFS where nodes and data are addressed using unique cryptographic hashes. Overall routing is implemented using Distributed Hash Tables (DHTs), and which can be used to find and publish data for peers. The proposed architecture is defined in Figure \ref{mural1}. These DHTs can store data within the network, and can thus reduce the latency in accessing data. A Merkle DAG along with Git versioning keeps the infrastructure up-to-date. For security, IPFS uses secure file sharing and encrypted communication.

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.95\linewidth]{figures/mural1.gif}
\caption{Proposed IoT-IPFS architecture \cite{muralidharan2019interplanetary}}
\label{mural1}
\end{center}
\end{figure}

Nizamuddin et al  \cite{nizamuddin2019decentralized} implemented an IPFS infrastructure using Ethereum. They have documented their Solidity smart contracts on GitHub \cite{gitNizamuddin} and tested them under Remix - an Ethereum IDE (Integrated Development Environment) which allows for development of smart contracts \cite{remix2021}. Figure \ref{niz02} outlines the implementation of the smart contract and which defines Developers (D) and Approvers (A). These are identified by Ethereum addresses, and where the creator of a document creates one smart contract for each document. Developers are then responsible in uploading the document (off-chain) to the IPFS file system.   The system requires a two-thirds majority of new developers/approvers to be approved by existing approvers (Figure \ref{naz03}). 

\begin{figure}
\begin{center}
\includegraphics[width=0.95\linewidth]{figures/naz03.jpg}
\caption{Document approval sequence approval \cite{nizamuddin2019decentralized}}
\label{naz03}
\end{center}
\end{figure}

\subsubsection{Performance}
Henningsten et al \cite{henningsen2020mapping} measured the performance of IPFS and used a  Kademlia-based distributed hash table (DHT). They had an average of 44,474 nodes of which  52.19\% resided behind a NAT. They found that the infrastructure was robust and was resistance against Sybil attacks. Unfortunately they identified weaknesses related to performance and in the privacy of queries.

\begin{figure}
\begin{center}
\includegraphics[width=0.95\linewidth]{figures/ipfs02.jpg}
\caption{Ethereum smart contract-based system for controlled document sharing \cite{nizamuddin2019decentralized}}
\label{niz02}
\end{center}
\end{figure}


Naz et al \cite{naz2019secure} implements a data sharing model (Figure \ref{naz01}) with a number of entities:

\begin{itemize}
\item Owner. This relates to the entity who is sharing the data, such as a government entity. 
\item Customer. This relates to an entity which can download files from an IPFS server using reconstructed hashes.
\item Workers. These help customers to de-crypt content, authenticate new customers through signatures, and query smart contracts customer data requests. 
\item Arbitrator. This entity resolves disputes between buyers and sellers for requested content.
\end{itemize}

With Naz's model \cite{naz2019secure}, an owner creates meta data for a file they wish to share, such as for filename, file type, file size, and a description. This information, and a complete copy of the file data, is then added to the IPFS. An example is (\cite{naz2019secure}):

\begin{lstlisting}[language=javascript]
//upload the plain file meta
ipfs.files.add(buf, function (err, meta_result) {
      if(err) {
                console.log(err);
                return res.sendStatus(500);
                }
                console.log(meta_result);
                res.json({ "meta_hash": meta_result[0].hash,
                "file_hash": fileMeta.hash,
                "address": recipient_addr,
                "email": recipient_email });
          }:
\end{lstlisting}

\begin{figure}
\begin{center}
\includegraphics[width=0.95\linewidth]{figures/naz01.png}
\caption{Data sharing on IPFS \cite{naz2019secure}}
\label{naz01}
\end{center}
\end{figure}

Once loaded onto the IPFS, the owner receives the hashes of the data back, who then contacts trusted worker nodes. These worker nodes have their key-pairs stored within smart contracts, and are responsible for decrypting content. The file hashes are split into $k$ shares using the Shamir Secret Share (SSS) method, and encrypted using $n$ random keys. These shares are then stored - along with security information -  on a blockchain. It is important to encrypt these hashes as an adversary could rebuild the file based on the hashes. Only valid customers who have paid for access, can then rebuild the files. A share for $S$ can then be {$S_1$, ... ,$S_n$} shares, and where there are $n$ shares and  a threshold of $k$. Overall $k$ shares are required to rebuild the secret. These shares are stored and encrypted in a smart contact and can only be decrypted and rebuild by verified workers (who are found by their public key by the owner).


Ali et al \cite{ali2017iot} used a side-chain method to keep network privacy and where a validator node runs the side chain (Figure \ref{side1}). Within the network, each IoT device has public and private keys and which they use to encrypt data for the validator. The validator then adds data onto a side chain. A smart contact then stores that the only communication is between the device and the validator. It also stores the public key and hash of the IPFS storing data on a device, and the public key and access rights of requesters from the consortium.  



\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.95\linewidth]{figures/side.png}
\caption{Side-chain method \cite{ali2017iot}}
\label{side1}
\end{center}
\end{figure}


Kumar et al \cite{kumar2019implementation} outlined a way to implement IPFS networks in order to reduce transaction size of block in the  blockchain, and a content-addressed based access of transactions. With this, miners store transactions on the IPFS distributed system storage. They then get back the IPFS hash of transaction and store in a block on the blockchain. Their experimental setup can be seen in Figure~\ref{kumar}.

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.95\linewidth]{figures/p246-kumar-fig-1-source-large.gif}
\caption{Working model of blockchain and IPFS  \cite{kumar2019implementation}}
\label{kumar}
\end{center}
\end{figure}

\subsubsection{Applications}

Sun et al \cite{sun2020blockchain} used a ciphertext policy attribute-based encryption (CP-ABE) and IPFS to securely store and sharing of electronic medical records. CP-ABE to control the access to encrypted files, and IPFS then stores these in a distributed form.  Figure \ref{fig:sun2020blockchain} provides an overview of the system and which is made up of: Blockchain, IPFS, medical system, and data user (DU). In this case CP-ABE is use to generate an encryption key based on a policy which is made-up from a number of attributes. A workflow is \cite{sun2020blockchain} :

\begin{itemize}
\item Initially a public-private key pair is created for Bob (the patient) based on his attributes. Bob then goes to hospital and doctor Alice diagnoses a condition.  
\item Alice encrypts the diagnosis (R) with Bob's public key (CT) and signs the diagnosis ( $CT' = (CT , sig_R$)). She then uploads to IPFS and generates an index for keywords. The IFPS returns a hash address (HASHID) for the file ($h$).
\item On receipt of the hash address, the Alice encrypts $h$ with a random number, and hashes the medical records and its index with SHA256. The hash value ($h_R$) and the encrypted hash ($h'$) are then stored on the blockchain by broadcasting the transaction. $h_R$ is the hash value of the record, and $h'$ is the encrypted hash address.
\item A transaction ID (TRANSID) is then returned from the blockchain. 
\end{itemize}

To recall the record:

\begin{itemize}
\item Bob sends an access request with keywords to the hospital. If he has rights of access, a search token is returned ($ST_w = (ID,h,\gamma$).
\item Bob veriﬁes the hash address $h$ which contains in the search token $ST_w$, and downloads the encrypted medical record (CT') using the IPFS for hash address $h$. 
\item Bob decrypts the ciphertext with his private key and obtains the file. 
\end{itemize}

The advantages of this scheme is that Bob needs to be authorized to gain access to private data, and needs to be authorized. The weaknesses of the system include its inability to revoke attributes for access and expired users \cite{sun2020blockchain}. 



\begin{figure}[h!]
%\begin{center}
\centering
\includegraphics[width=0.9\linewidth]{figures/yao1-2982964-large.gif}
\caption{Health care storage in IPFS  \cite{sun2020blockchain}}
\label{fig:sun2020blockchain}
%\end{center}
\end{figure}



Taborda et al \cite{taborda2020decentralized} have created a Web platform to store information on hotels for an image repository. This uses IPFS and blockchain in order to improve security and access control. Hao et al \cite{hao2018safe} define a data storage system which uses IPFS to store video, images, and real-time monitoring data reported from sensors in agricultural products tracking (Figure \ref{arg}).  

Nizamuddin \cite{nizamuddin2018ipfs} defines an IPFS/smart contract solution to prove the originality and authenticity of published work and digital content. They use Ethereum smart contracts in order to govern, manage, and provide traceability and visibility of the history of digital content from its original version to the current version. In the work they create a use case of an online book publication (Figure \ref{book}). Figure \ref{book2} outlines the message sequence diagram for validation. 

Vishwavidyapeetham et al \cite{vishwavidyapeetham2018blockchain} apply IPFS to making notes within research projects. It uses a traditional encryption method to create a secure documents for record keeping and  Ethereum smart contracts to track the encrypted files.

Patsakis \cite{patsakis2019hydras}.
define Resource Identiﬁer Generation Algorithms and which extend Domain Generation Algorithms (DGA) - and which are often used by cybercriminals for bot management and communication. Their system extends beyond DNS to use IPFS. overall it hosts malicious content and explores ways that a botmaster deploys and controls bots. Figure \ref{bot} provides an overview of the system.

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.95\linewidth]{figures/arg.png}
\caption{Agricultural products tracking  \cite{taborda2020decentralized}}
\label{arg}
\end{center}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.95\linewidth]{figures/book.png}
\caption{Book tracking system  \cite{nizamuddin2018ipfs}}
\label{book}
\end{center}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.95\linewidth]{figures/book2.png}
\caption{Smart contract tracking system  \cite{nizamuddin2018ipfs}}
\label{book2}
\end{center}
\end{figure}


\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.95\linewidth]{figures/pi.png}
\caption{Record keeping system on IPFS   \cite{vishwavidyapeetham2018blockchain}}
\label{pi}
\end{center}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.95\linewidth]{figures/bot.png}
\caption{Hydras and IPFS: a decentralised playground for malware   \cite{patsakis2019hydras}}
\label{bot}
\end{center}
\end{figure}


Karapapas et al \cite{karapapas2020ransomware} define that decentralized systems provide opportunities for cybercriminals to perform illegal activities. A scenario for this is defined in Figure \ref{ransom}.

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.95\linewidth]{figures/ransom.png}
\caption{Ransomware on IPFS \cite{karapapas2020ransomware}}
\label{ransom}
\end{center}
\end{figure}

Overall Nizamuddin et al \cite{nizamuddin2019decentralized} define a number of drivers for a business model using cryptocurrencies. With its integrated version control systems, the infrastructure will enable tamper-proof version control. 

\section{GLASS Architecture}
GLASS thus aims to create new models for digital governance, and which supports the integration of targeted, engaging and effective policies for the citizen. This will focus a range of key technologies including Distributed Ledgers, Big Data Analytics, Machine Learning, Artificial Intelligence, AIBots and NetApps technologies, and aim for a digital-by-default design, and which support interoperable and cross-border integration. The overall architecture is defined in Figure \ref{glass02}.

\begin{center}
\begin{figure*}
\begin{center}
\includegraphics[width=0.95\linewidth]{figures/glass02.png}
\label{glass02}
\caption{GLASS Architecture\cite{glass2021}}
\end{center}
\end{figure*}
\end{center}
